Real-Time Online Skeleton Extraction and Gesture Recognition on Pepper

We present a multi-stage pipeline for simple gesture recognition. The novelty of our approach is the association of different technologies, resulting in the first real-time system as of now to conjointly extract skeletons and recognise gesture on a Pepper robot. For this task, Pepper has been augmented with an embedded GPU for running deep CNNs and a fish-eye camera to capture whole scene interaction. We show in this article that real-case scenarios are challenging, and the state-of-the-art approaches hardly deal with unknown human gestures. We present here a way to handle such cases.

==> sec_tracker.tex <==
\section{\uppercase{human tracker}}
\label{sec:tracker}

Our motivation in this section is the development of a real-time multi-human tracker \cite{tracker_1}\cite{tracker_2} to identify the movement of every detected humans in the scene. This tracking step is useful for the gesture recognition, in case there are multiple persons in the frame, to avoid mixing their skeletons as Openpose has a non-deterministic detection order.

The tracking is reduced to an association task, consisting of determining what detection, i.e. new skeletons, corresponds to what subject, based on the location of the subjects at the previous time-step. Also, in a complex scene, people may leave (less measurements than currently tracked objects) or enter the scene (more measurements than currently tracked objects). 

This task of matching every detection to every already tracked object can be formulated as the assignment problem, a combinatorial optimisation problems consisting of finding an optimal matching between two sets, the measurements (or new detection) $M$ and the objects (already tracked people) $O$. 

There is a cost $c_{ij}$ assigning a measurement $m$ to an object $o$, that it the similarity between the new detection and the already tracked subjects. Given the body-joints location of every humans, different similarity measures can be computed, such as the intersection over union (IoU) of the bounding box encompassing the skeletons, or the euclidean distance of the joints location (e.g. OKS metric). 

Given this weighted graph, the maximum matching can be obtained with the Hungarian algorithm \cite{hungarian}. The Hungarian algorithm has a linear time complexity of $\mathcal{O}(n^3)$, which allow fast matching for small-scale tracking, although it doesn't scale for large number of people in a video.

This tracking approach still suffers from several limitations. The detections are usually noisy, meaning that joints may be wrongly located or labelled, and in the case of a \textit{bottom-up} detector, assigned to the wrong human. Probabilistic predictors like the Kalman filter \cite{kalman_filter} or the particle filter \cite{particle_filter} should correct this issue as they naturally incorporate the problem of noisy detection in their design. Another inconvenient issue is the impossibility to track people while the robot, specifically the camera, is moving. The body-parts location are measured in the camera frame, and thus are not rectified when the camera moves. The ideal solution would be to estimate the joints in the world frame \cite{densepose}.
